Multi-task Supervised Learning via Cross-learning

In this paper we consider a problem known as multi-task learning, consisting of fitting a set of classifier or regression functions intended for solving different tasks. In our novel formulation, we couple the parameters of these functions, so that they learn in their task specific domains while staying close to each other. This facilitates cross-fertilization in which data collected across different domains help improving the learning performance at each other task. First, we present a simplified case in which the goal is to estimate the means of two Gaussian variables, for the purpose of gaining some insights on the advantage of the proposed cross-learning strategy. Then we provide a stochastic projected gradient algorithm to perform cross-learning over a generic loss function. If the number of parameters is large, then the projection step becomes computationally expensive. To avoid this situation, we derive a primal-dual algorithm that exploits the structure of the dual problem, achieving a formulation whose complexity only depends on the number of tasks. Preliminary numerical experiments for image classification by neural networks trained on a dataset divided in different domains corroborate that the cross-learned function outperforms both the task-specific and the consensus approaches.

==> fig/fig_epsilons.tex <==

\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}

	\begin{semilogxaxis}[
		tick scale binop=\times,
		minor tick num=1,
		xlabel={Centrality ($\epsilon$)},
		ylabel={Accuracy ($\%$)},
		ylabel near ticks,
		width=\columnwidth, 
		ytick={0,10,20,30,40,50},
        xtick={0.000001,0.00001,0.0001,0.001,0.01,0.1},
        xticklabels={$0$,$10^{-5}$,$10^{-4}$,$10^{-3}$,$10^{-2}$,$10^{-1}$}, 			
		height=0.6\columnwidth, 
		xmin=0.000001,xmax=0.1,ymin=0,ymax=50,
		grid=both,
		axis line style={draw=none},
		legend style={
			at={(0,1.06)}, 
			anchor=south west, 
			legend cell align=left,
			legend columns=4
		}		
	]
	
%Cross-Learning
	\addplot [color=red,mark=*,mark options={fill=red,scale=0.5, color =red},solid,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{art}] {fig/data/NN_epsilons.dat};
	\addlegendentry{Art};
	
	\addplot [color=blue,mark=*,mark options={fill=blue,scale=0.5, color =blue},solid,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{clipart}] {fig/data/NN_epsilons.dat};
	\addlegendentry{Clipart};

	\addplot [color=green,mark=*,mark options={fill=green,scale=0.5, color =green},solid,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{product}] {fig/data/NN_epsilons.dat};
	\addlegendentry{Product};

	\addplot [color=black,mark=*,mark options={fill=black,scale=0.5, color =black},solid,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{real world}] {fig/data/NN_epsilons.dat};
	\addlegendentry{Real World};


%Agnostic
	\addplot [color=red,dashed,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{art}] {fig/data/NN_agnostic.dat};

	\addplot [color=blue,dashed,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{clipart}] {fig/data/NN_agnostic.dat};
	
	\addplot [color=green,dashed,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{product}] {fig/data/NN_agnostic.dat};

\addplot [color=black,dashed,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{real world}] {fig/data/NN_agnostic.dat};

%Consensus Line
\addplot [color=red, dotted,thick] 
	table[col sep=comma, x index=0,y expr=\thisrow{art}] {fig/data/NN_consensus_line.dat};
\addplot [color=blue, dotted,thick] 
	table[col sep=comma, x index=0,y expr=\thisrow{clipart}] {fig/data/NN_consensus_line.dat};
\addplot [color=green, dotted,thick] 
	table[col sep=comma, x index=0,y expr=\thisrow{product}] {fig/data/NN_consensus_line.dat};
\addplot [color=black, dotted,thick] 
	table[col sep=comma, x index=0,y expr=\thisrow{real world}] {fig/data/NN_consensus_line.dat};

\end{semilogxaxis}

	\begin{axis}[
		axis x discontinuity=crunch,
		xlabel={Centrality ($\epsilon$)},
		ylabel={Accuracy ($\%$)},
		ylabel near ticks,
		width=\columnwidth, 
		ytick={0,10,20,30,40,50},
        xtick={0.000001,0.00001,0.0001,0.001,0.01,0.1},
        xticklabels={,,},
        ytick style={draw=none},
        xtick style={draw=none},
		height=0.6\columnwidth, 
		xmin=0.000001,xmax=0.1,ymin=0,ymax=50,
		grid=none
	]

%Initial Dot (Consensus)
\addplot [color=red, only marks, mark=*] 
	table[col sep=comma, x index=0,y expr=\thisrow{art}] {fig/data/NN_consensus_dot.dat};
\addplot [color=blue, only marks, mark=*] 
	table[col sep=comma, x index=0,y expr=\thisrow{clipart}] {fig/data/NN_consensus_dot.dat};
\addplot [color=green, only marks, mark=*] 
	table[col sep=comma, x index=0,y expr=\thisrow{product}] {fig/data/NN_consensus_dot.dat};
\addplot [color=black, only marks, mark=*] 
	table[col sep=comma, x index=0,y expr=\thisrow{real world}] {fig/data/NN_consensus_dot.dat};

%Final Dot (Cross-Learning)
	\addplot [color=red,mark=*,mark options={fill=red,scale=0.5, color =red},solid,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{art}] {fig/data/NN_epsilons_dot.dat};
	
	\addplot [color=blue,mark=*,mark options={fill=blue,scale=0.5, color =blue},solid,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{clipart}] {fig/data/NN_epsilons_dot.dat};

	\addplot [color=green,mark=*,mark options={fill=green,scale=0.5, color =green},solid,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{product}] {fig/data/NN_epsilons_dot.dat};

	\addplot [color=black,mark=*,mark options={fill=black,scale=0.5, color =black},solid,thick] 
		table[col sep=comma, x index=0,y expr=\thisrow{real world}] {fig/data/NN_epsilons_dot.dat};

\end{axis}	


\end{tikzpicture}


==> latex_resources/plot_appearance.tex <==


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\tiny},   % Write numbers in tiny font
              label style = {font=\tiny},        % Write axes labels in tiny size font
              title style = {font=\tiny},        % Write figure titles in tiny size font
            }

% style to draw dots in comb plots 
\tikzstyle{dot}          =[circle, draw=none, inner sep=0pt, minimum size =1.5mm, fill=black]
\tikzstyle{red dot}      =[dot, fill=red]
\tikzstyle{blue dot}     =[dot, fill=blue ]
\tikzstyle{red blue dot} =[dot, draw, thick, minimum size =1.2mm, red, fill=blue]
\def \greenfill {mygreen!40}
